Lottery Ticket Preserves Weight Correlation: Is It Desirable or Not?

In deep model compression, the recent finding "Lottery Ticket Hypothesis" (LTH) (Frankle & Carbin, 2018) pointed out that there could exist a winning ticket (i.e., a properly pruned sub-network together with original weight initialization) that can achieve competitive performance than the original dense network. However, it is not easy to observe such winning property in many scenarios, where for example, a relatively large learning rate is used even if it benefits training the original dense model. In this work, we investigate the underlying condition and rationale behind the winning property, and find that the underlying reason is largely attributed to the correlation between initialized weights and final-trained weights when the learning rate is not sufficiently large. Thus, the existence of winning property is correlated with an insufficient DNN pretraining, and is unlikely to occur for a well-trained DNN. To overcome this limitation, we propose the "pruning & fine-tuning" method that consistently outperforms lottery ticket sparse training under the same pruning algorithm and the same total training epochs. Extensive experiments over multiple deep models (VGG, ResNet, MobileNet-v2) on different datasets have been conducted to justify our proposals.

==> figs-rebuttal/fig_top10overlap.tex <==
\vspace{-10pt}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\columnwidth]{figs-rebuttal/top10overlap_new.pdf}
    \vspace{-13pt}
    \caption{Overlap ratios (p=10\%) between the pre-trained weights $\theta_T$ and weights on each training epoch $\theta_t, t \in [0,T]$ for pre-training of ResNet-20 on CIFAR-10 at lr of 0.01 and 0.1.}
    \label{fig:reb_overlap}
\end{figure}

==> figs-rebuttal/table_RNN.tex <==
% % \setlength{\textfloatsep}{4pt}
% \begin{table}[t]
% \scriptsize\sffamily
% % \footnotesize\sffamily
%     \centering
%     \renewcommand{\arraystretch}{1.2}
% \begin{adjustbox}{max width=1\columnwidth}
% \begin{tabular}{@{} l l *{1}{r} @{}}
% \toprule
% \bfseries 
% \bfseries \begin{tabular}{@{}l@{}}Model\end{tabular}
% & \bfseries \begin{tabular}{@{}r@{}}Learning rate\end{tabular}
% & \bfseries \begin{tabular}{@{}r@{}}Word error rate\end{tabular}
% % \\[2ex]
%     \toprule
%     % \multicolumn{3}{c}{\textbf{Scale $\times 2$}} \\ 
%     % \midrule
%     % \midrule
%     % \multirow{11}{*}{\rotatebox[origin=c]{0}{\footnotesize $\times$ 2}}
%     \textsc{SRCNN} &  57 & 52.7\\
%     % \midrule
%     % \multicolumn{6}{c}{\textbf{Scale $\times 4$}} \\ 
%     \midrule
%     \textsc{SRCNN} & 57 & 52.7\\

%     \bottomrule

% \end{tabular}
% \end{adjustbox}
%     \caption{Comparison with state-of-the-art efficient SR models.}
%         \label{table:result_sr}
% % \vspace{-4mm}
% \end{table}


% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \vspace{-20pt}
\begin{table}[h]
\vspace{-18pt}
\caption{Results of more datasets and applications.}
\centering
% \footnotesize
\begin{adjustbox}{max width=0.9\columnwidth}
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{5}{|c|}{\textbf{Image classification: ResNet50 on ImageNet dataset with 90\% sparsity}} \\ \hline
Model & Learning Rate & Pretrained & Top-1 Acc. & Overlap Ratio \\ \hline
prune \& finetune & \multirow{3}{*}{4e-1} & \multirow{3}{*}{76.1\%} & 75.3\% & - \\ \cline{1-1} \cline{4-5} 
``Winning ticket'' &  &  & 70.5\% & \multirow{2}{*}{10.3\%} \\ \cline{1-1} \cline{4-4}
Random reinit &  &  & 70.3\% &  \\ \hline
prune \& finetune & \multirow{3}{*}{4e-2} & \multirow{3}{*}{72.4\%} & 71.1\% & - \\ \cline{1-1} \cline{4-5} 
``Winning ticket'' &  &  & 66.5\% & \multirow{2}{*}{25.5\%} \\ \cline{1-1} \cline{4-4}
Random reinit &  &  & 65.6\% &  \\ \hline
\multicolumn{5}{|c|}{\textbf{Automatic speech recognition: GRU on TIMIT dataset with 90\% sparsity}} \\ \hline
Model & Learning Rate & Pretrained & WER & Overlap Ratio \\ \hline
prune \& finetune & \multirow{3}{*}{4e-4} & \multirow{3}{*}{18.8\%} & 18.9\% & - \\ \cline{1-1} \cline{4-5} 
``Winning ticket'' &  &  & 20.8\% & \multirow{2}{*}{19.8\%} \\ \cline{1-1} \cline{4-4}
Random reinit &  &  & 20.9\% &  \\ \hline
prune \& finetune & \multirow{3}{*}{4e-5} & \multirow{3}{*}{24.6\%} & 24.2\% & - \\ \cline{1-1} \cline{4-5} 
``Winning ticket'' &  &  & 24.6\% & \multirow{2}{*}{51.2\%} \\ \cline{1-1} \cline{4-4}
Random reinit &  &  & 25.5\% &  \\ \hline
\multicolumn{5}{|c|}{\textbf{Object detection: YOLOv4 on MS-COCO dataset with 87.5\% sparsity}} \\ \hline
Model & Learning Rate & Pretrained & mAP & Overlap Ratio \\ \hline
prune \& finetune & \multirow{3}{*}{1e-3} & \multirow{3}{*}{57.3\%} & 54.1\% & - \\ \cline{1-1} \cline{4-5} 
``Winning ticket'' &  &  & 42.3\% & \multirow{2}{*}{13.1\%} \\ \cline{1-1} \cline{4-4}
Random reinit &  &  & 42.4\% &  \\ \hline
\end{tabular}
\end{adjustbox}
\label{table:rnn}
\vspace{-5pt}
\end{table}

% ``prune \& finetune''
% ``Winning ticket''



% % % Please add the following required packages to your document preamble:
% % % \usepackage{multirow}
% \begin{table}[h]
% \caption{Results on RNN using GRU on TIMIT dataset.}
% \centering
% % \footnotesize
% \begin{adjustbox}{max width=0.9\columnwidth}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% Model & \begin{tabular}[c]{@{}c@{}}Learning\\ Rate (LR)\end{tabular} & 
% \begin{tabular}[c]{@{}c@{}}Pretrained\\WER\end{tabular} & NLLLoss & \begin{tabular}[c]{@{}c@{}}Word Error\\ Rate (WER)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Overlap\\ Ratio\end{tabular} \\ \hline
% ``prune \& finetune'' & \multirow{3}{*}{4e-4} & \multirow{3}{*}{18.8} & 1.017 & 18.9 & - \\ \cline{1-1} \cline{4-6} 
% ``Winning ticket'' &  &  & 1.159 & 20.8 & \multirow{2}{*}{25.9\%} \\ \cline{1-1} \cline{4-5}
% Random reinit &  &  & 1.661 & 21.0 &  \\ \hline
% ``prune \& finetune'' & \multirow{3}{*}{4e-5} & \multirow{3}{*}{24.6} & 2.411 & 24.2 & - \\ \cline{1-1} \cline{4-6} 
% ``Winning ticket'' &  &  & 2.928 & 24.6 & \multirow{2}{*}{51.2\%} \\ \cline{1-1} \cline{4-5}
% Random reinit &  &  & 3.641 & 25.5 &  \\ \hline
% \end{tabular}
% \end{adjustbox}
% \label{table:rnn}
% \end{table}
